Retrieval Study of Brown Dwarfs Across the L-T Sequence

A large suite of 228 atmospheric retrievals is performed on a curated sample of 19 brown dwarfs spanning the L0 to T8 spectral types using the open-source Helios-r2 retrieval code, which implements the method of short characteristics for radiative transfer and a finite-element description of the temperature-pressure profile. Surprisingly, we find that cloud-free and cloudy (both gray and non-gray) models are equally consistent with the archival SpeX data from the perspective of Bayesian model comparison. Only upper limits for cloud properties are inferred if log-uniform priors are assumed, but the cloud optical depth becomes constrained if a uniform prior is used. Water is detected in all 19 objects and methane is detected in all of the T dwarfs, but no obvious trend exists across effective temperature. As carbon monoxide is only detected in a handful of objects, the inferred carbon-to-oxygen ratios are unreliable. The retrieved radius generally decreases with effective temperature, but the values inferred for some T dwarfs are implausibly low and may indicate missing physics or chemistry in the models. For the early L dwarfs, the retrieved surface gravity depends on whether the gray or non-gray cloud model is preferred. Future data are necessary for constraining cloud properties and the vertical variation of chemical abundances, the latter of which is needed for distinguishing between the chemical instability versus traditional cloud interpretation of the L-T transition.

==> tables_single.tex <==


\begin{table*}%[!h]
\label{tab:log g entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	$	3.73^{+0.12}_{-0.13} 	$	& 	$	4.75^{+0.13}_{-0.14} 	$	& 	$	6.42^{+0.08}_{-0.06} 	$	& 	& 	$	5.10^{+0.31}_{-0.14} 	$	& 	$	5.10^{+0.29}_{-0.14} 	$	& 	$	5.85^{+0.36}_{-0.37} 	$	\\
L1 	& 	$	4.15^{+0.17}_{-0.16} 	$	& 	$	4.16^{+0.17}_{-0.15} 	$	& 	$	5.02^{+0.13}_{-0.20} 	$	& 	& 	$	5.00^{+0.34}_{-0.21} 	$	& 	$	4.98^{+0.37}_{-0.22} 	$	& 	$	5.60^{+0.44}_{-0.26} 	$	\\
L2 	& 	$	4.29^{+0.42}_{-0.64} 	$	& 	$	5.00^{+0.15}_{-0.12} 	$	& 	$	6.21^{+0.27}_{-0.20} 	$	& 	& 	$	4.95^{+0.33}_{-0.20} 	$	& 	$	5.03^{+0.29}_{-0.15} 	$	& 	$	6.10^{+0.50}_{-0.27} 	$	\\
L3 	& 	$	5.29^{+0.10}_{-0.06} 	$	& 	$	5.07^{+0.17}_{-0.17} 	$	& 	$	6.23^{+0.29}_{-0.18} 	$	& 	& 	$	5.13^{+0.17}_{-0.14} 	$	& 	$	5.14^{+0.16}_{-0.14} 	$	& 	$	5.29^{+0.20}_{-0.28} 	$	\\
L4 	& 	$	4.63^{+0.54}_{-0.46} 	$	& 	$	4.67^{+0.54}_{-0.44} 	$	& 	$	5.30^{+0.68}_{-0.46} 	$	& 	& 	$	4.86^{+0.52}_{-0.32} 	$	& 	$	4.87^{+0.52}_{-0.33} 	$	& 	$	5.77^{+0.64}_{-0.42} 	$	\\
L5 	& 	$	5.67^{+0.14}_{-0.12} 	$	& 	$	5.35^{+0.15}_{-0.14} 	$	& 	$	5.61^{+0.23}_{-0.21} 	$	& 	& 	$	5.58^{+0.15}_{-0.14} 	$	& 	$	5.58^{+0.14}_{-0.14} 	$	& 	$	6.19^{+0.25}_{-0.20} 	$	\\
L6 	& 	$	5.15^{+0.48}_{-0.35} 	$	& 	$	5.21^{+0.46}_{-0.31} 	$	& 	$	5.80^{+0.62}_{-0.45} 	$	& 	& 	$	5.18^{+0.38}_{-0.31} 	$	& 	$	5.19^{+0.44}_{-0.29} 	$	& 	$	6.02^{+0.61}_{-0.31} 	$	\\
L7 	& 	$	4.63^{+0.63}_{-0.53} 	$	& 	$	4.73^{+0.56}_{-0.44} 	$	& 	$	5.43^{+0.54}_{-0.36} 	$	& 	& 	$	4.31^{+0.48}_{-0.63} 	$	& 	$	4.36^{+0.48}_{-0.57} 	$	& 	$	4.59^{+0.60}_{-1.02} 	$	\\
L8 	& 	$	5.40^{+0.18}_{-0.17} 	$	& 	$	5.38^{+0.18}_{-0.17} 	$	& 	$	5.71^{+0.24}_{-0.19} 	$	& 	& 	$	5.25^{+0.27}_{-0.20} 	$	& 	$	5.25^{+0.27}_{-0.19} 	$	& 	$	5.88^{+0.44}_{-0.46} 	$	\\
L9 	& 	$	5.59^{+0.07}_{-0.06} 	$	& 	$	5.28^{+0.15}_{-0.17} 	$	& 	$	5.56^{+0.17}_{-0.15} 	$	& 	& 	$	5.62^{+0.14}_{-0.08} 	$	& 	$	5.28^{+0.17}_{-0.17} 	$	& 	$	5.65^{+0.13}_{-0.12} 	$	\\
T0 	& 	$	4.36^{+0.32}_{-0.89} 	$	& 	$	4.27^{+0.24}_{-0.32} 	$	& 	$	4.26^{+0.25}_{-0.45} 	$	& 	& 	$	4.06^{+0.19}_{-0.25} 	$	& 	$	4.05^{+0.18}_{-0.20} 	$	& 	$	4.04^{+0.16}_{-0.18} 	$	\\
T1 	& 	$	4.46^{+0.07}_{-0.07} 	$	& 	$	4.48^{+0.08}_{-0.09} 	$	& 	$	4.47^{+0.07}_{-0.07} 	$	& 	& 	$	4.50^{+0.10}_{-0.15} 	$	& 	$	4.45^{+0.08}_{-0.09} 	$	& 	$	4.48^{+0.08}_{-0.09} 	$	\\
T2 	& 	$	3.72^{+0.08}_{-0.08} 	$	& 	$	3.93^{+0.24}_{-0.22} 	$	& 	$	3.76^{+0.11}_{-0.24} 	$	& 	& 	$	3.71^{+0.11}_{-0.12} 	$	& 	$	3.72^{+0.11}_{-0.12} 	$	& 	$	3.71^{+0.10}_{-0.11} 	$	\\
T3 	& 	$	5.36^{+0.12}_{-0.12} 	$	& 	$	5.38^{+0.13}_{-0.14} 	$	& 	$	5.38^{+0.12}_{-0.13} 	$	& 	& 	$	5.37^{+0.11}_{-0.11} 	$	& 	$	5.41^{+0.13}_{-0.21} 	$	& 	$	5.35^{+0.10}_{-0.08} 	$	\\
T4 	& 	$	3.72^{+0.10}_{-0.10} 	$	& 	$	3.75^{+0.11}_{-0.18} 	$	& 	$	3.74^{+0.09}_{-0.09} 	$	& 	& 	$	4.36^{+0.23}_{-0.26} 	$	& 	$	4.37^{+0.22}_{-0.24} 	$	& 	$	4.37^{+0.20}_{-0.23} 	$	\\
T5 	& 	$	4.83^{+0.10}_{-0.11} 	$	& 	$	4.83^{+0.10}_{-0.11} 	$	& 	$	4.82^{+0.09}_{-0.11} 	$	& 	& 	$	4.73^{+0.13}_{-0.14} 	$	& 	$	4.73^{+0.13}_{-0.13} 	$	& 	$	4.73^{+0.12}_{-0.12} 	$	\\
T6 	& 	$	4.61^{+0.25}_{-0.25} 	$	& 	$	4.60^{+0.24}_{-0.24} 	$	& 	$	4.60^{+0.23}_{-0.24} 	$	& 	& 	$	4.53^{+0.52}_{-0.32} 	$	& 	$	4.53^{+0.46}_{-0.30} 	$	& 	$	4.56^{+0.42}_{-0.27} 	$	\\
T7 	& 	$	4.92^{+0.13}_{-0.16} 	$	& 	$	4.91^{+0.12}_{-0.15} 	$	& 	$	4.59^{+0.15}_{-0.17} 	$	& 	& 	$	3.91^{+0.17}_{-0.20} 	$	& 	$	3.82^{+0.14}_{-0.16} 	$	& 	$	3.91^{+0.16}_{-0.18} 	$	\\
T8 	& 	$	3.67^{+0.10}_{-0.12} 	$	& 	$	3.67^{+0.10}_{-0.12} 	$	& 	$	3.67^{+0.10}_{-0.11} 	$	& 	& 	$	3.66^{+0.10}_{-0.16} 	$	& 	$	3.67^{+0.10}_{-0.15} 	$	& 	$	4.08^{+0.42}_{-0.64} 	$	\\
\hline
\hline
\end{tabular} }\\
\end{table*}


\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:R entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	$1.33^{+0.07}_{-0.08}$ 	& 	$1.25^{+0.05}_{-0.05}$ 	& 	$1.64^{+0.11}_{-0.11}$ 	& 	& 	$1.00^{+0.05}_{-0.04}$ 	& 	$1.00^{+0.05}_{-0.04}$ 	& 	$0.95^{+0.03}_{-0.04}$ 	\\
L1 	& 	$1.14^{+0.05}_{-0.05}$ 	& 	$1.14^{+0.05}_{-0.05}$ 	& 	$1.23^{+0.04}_{-0.04}$ 	& 	& 	$1.00^{+0.03}_{-0.03}$ 	& 	$1.01^{+0.03}_{-0.03}$ 	& 	$0.99^{+0.03}_{-0.03}$ 	\\
L2 	& 	$1.12^{+0.06}_{-0.09}$ 	& 	$1.15^{+0.05}_{-0.05}$ 	& 	$1.14^{+0.05}_{-0.05}$ 	& 	& 	$1.07^{+0.04}_{-0.04}$ 	& 	$1.07^{+0.04}_{-0.04}$ 	& 	$1.04^{+0.03}_{-0.03}$ 	\\
L3 	& 	$0.93^{+0.03}_{-0.03}$ 	& 	$0.94^{+0.03}_{-0.03}$ 	& 	$0.98^{+0.04}_{-0.05}$ 	& 	& 	$0.94^{+0.03}_{-0.03}$ 	& 	$0.94^{+0.03}_{-0.03}$ 	& 	$0.93^{+0.03}_{-0.03}$ 	\\
L4 	& 	$0.97^{+0.14}_{-0.13}$ 	& 	$0.96^{+0.14}_{-0.13}$ 	& 	$0.97^{+0.13}_{-0.11}$ 	& 	& 	$0.95^{+0.13}_{-0.12}$ 	& 	$0.94^{+0.12}_{-0.11}$ 	& 	$0.95^{+0.12}_{-0.10}$ 	\\
L5 	& 	$0.59^{+0.07}_{-0.10}$ 	& 	$0.77^{+0.10}_{-0.09}$ 	& 	$0.79^{+0.09}_{-0.08}$ 	& 	& 	$0.65^{+0.09}_{-0.11}$ 	& 	$0.66^{+0.09}_{-0.11}$ 	& 	$0.78^{+0.09}_{-0.07}$ 	\\
L6 	& 	$0.65^{+0.06}_{-0.06}$ 	& 	$0.65^{+0.06}_{-0.05}$ 	& 	$0.65^{+0.06}_{-0.05}$ 	& 	& 	$0.66^{+0.06}_{-0.06}$ 	& 	$0.69^{+0.06}_{-0.06}$ 	& 	$0.69^{+0.05}_{-0.05}$ 	\\
L7 	& 	$0.83^{+0.07}_{-0.07}$ 	& 	$0.86^{+0.07}_{-0.06}$ 	& 	$0.87^{+0.07}_{-0.07}$ 	& 	& 	$0.87^{+0.07}_{-0.08}$ 	& 	$0.86^{+0.07}_{-0.07}$ 	& 	$0.84^{+0.06}_{-0.07}$ 	\\
L8 	& 	$0.76^{+0.12}_{-0.14}$ 	& 	$0.76^{+0.12}_{-0.14}$ 	& 	$0.85^{+0.12}_{-0.11}$ 	& 	& 	$0.85^{+0.15}_{-0.18}$ 	& 	$0.85^{+0.14}_{-0.17}$ 	& 	$0.86^{+0.11}_{-0.11}$ 	\\
L9 	& 	$0.67^{+0.04}_{-0.03}$ 	& 	$0.63^{+0.02}_{-0.02}$ 	& 	$0.62^{+0.02}_{-0.02}$ 	& 	& 	$0.62^{+0.03}_{-0.03}$ 	& 	$0.61^{+0.02}_{-0.02}$ 	& 	$0.60^{+0.02}_{-0.02}$ 	\\
T0 	& 	$0.68^{+0.10}_{-0.10}$ 	& 	$0.69^{+0.10}_{-0.09}$ 	& 	$0.68^{+0.09}_{-0.09}$ 	& 	& 	$0.72^{+0.11}_{-0.10}$ 	& 	$0.72^{+0.10}_{-0.10}$ 	& 	$0.72^{+0.09}_{-0.09}$ 	\\
T1 	& 	$0.48^{+0.03}_{-0.03}$ 	& 	$0.48^{+0.03}_{-0.03}$ 	& 	$0.48^{+0.03}_{-0.03}$ 	& 	& 	$0.49^{+0.04}_{-0.04}$ 	& 	$0.50^{+0.04}_{-0.04}$ 	& 	$0.50^{+0.03}_{-0.04}$ 	\\
T2 	& 	$0.94^{+0.04}_{-0.05}$ 	& 	$0.93^{+0.04}_{-0.04}$ 	& 	$0.93^{+0.04}_{-0.04}$ 	& 	& 	$0.99^{+0.05}_{-0.06}$ 	& 	$0.99^{+0.06}_{-0.06}$ 	& 	$0.99^{+0.05}_{-0.05}$ 	\\
T3 	& 	$0.66^{+0.06}_{-0.06}$ 	& 	$0.66^{+0.06}_{-0.06}$ 	& 	$0.66^{+0.05}_{-0.06}$ 	& 	& 	$0.61^{+0.06}_{-0.06}$ 	& 	$0.60^{+0.06}_{-0.06}$ 	& 	$0.61^{+0.05}_{-0.06}$ 	\\
T4 	& 	$0.79^{+0.10}_{-0.10}$ 	& 	$0.79^{+0.10}_{-0.09}$ 	& 	$0.79^{+0.09}_{-0.09}$ 	& 	& 	$0.69^{+0.09}_{-0.09}$ 	& 	$0.68^{+0.09}_{-0.09}$ 	& 	$0.68^{+0.08}_{-0.08}$ 	\\
T5 	& 	$0.71^{+0.04}_{-0.04}$ 	& 	$0.71^{+0.04}_{-0.04}$ 	& 	$0.71^{+0.04}_{-0.04}$ 	& 	& 	$0.69^{+0.05}_{-0.05}$ 	& 	$0.69^{+0.05}_{-0.05}$ 	& 	$0.69^{+0.05}_{-0.05}$ 	\\
T6 	& 	$0.85^{+0.10}_{-0.11}$ 	& 	$0.86^{+0.09}_{-0.10}$ 	& 	$0.85^{+0.09}_{-0.09}$ 	& 	& 	$0.84^{+0.13}_{-0.15}$ 	& 	$0.84^{+0.12}_{-0.14}$ 	& 	$0.81^{+0.11}_{-0.12}$ 	\\
T7 	& 	$0.69^{+0.04}_{-0.04}$ 	& 	$0.69^{+0.04}_{-0.04}$ 	& 	$0.68^{+0.03}_{-0.03}$ 	& 	& 	$0.81^{+0.06}_{-0.06}$ 	& 	$0.86^{+0.06}_{-0.06}$ 	& 	$0.81^{+0.05}_{-0.06}$ 	\\
T8 	& 	$0.63^{+0.12}_{-0.13}$ 	& 	$0.63^{+0.12}_{-0.12}$ 	& 	$0.63^{+0.12}_{-0.12}$ 	& 	& 	$0.52^{+0.10}_{-0.11}$ 	& 	$0.53^{+0.10}_{-0.11}$ 	& 	$0.45^{+0.08}_{-0.11}$ 	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}


\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:Teff entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	$1799.16^{+48.86}_{-44.79}$ 	&	 $1852.63^{+38.11}_{-35.47}$ 	& 	$1619.61^{+53.75}_{-54.11}$ 	& 	& 	$1919.30^{+39.39}_{-47.06}$ 	&	 $1920.73^{+38.82}_{-48.32}$ 	& 	$1969.17^{+44.02}_{-33.88}$ 	\\
L1 	& 	$1873.90^{+39.95}_{-37.93}$ 	&	 $1874.60^{+38.86}_{-36.30}$ 	& 	$1804.20^{+29.53}_{-30.18}$ 	& 	& 	$1858.86^{+28.26}_{-28.95}$ 	&	 $1846.83^{+27.99}_{-27.14}$ 	& 	$1871.61^{+22.75}_{-24.09}$ 	\\
L2 	& 	$1730.29^{+62.21}_{-46.20}$ 	&	 $1709.85^{+37.96}_{-38.56}$ 	& 	$1719.26^{+33.55}_{-35.04}$ 	& 	& 	$1658.74^{+29.90}_{-30.73}$ 	&	 $1661.00^{+28.09}_{-30.66}$ 	& 	$1679.14^{+23.79}_{-26.02}$ 	\\
L3 	& 	$1674.93^{+28.44}_{-27.16}$ 	&	 $1660.35^{+26.88}_{-26.70}$ 	& 	$1626.62^{+39.43}_{-37.81}$ 	& 	& 	$1571.92^{+24.01}_{-23.91}$ 	&	 $1570.77^{+23.83}_{-23.23}$ 	& 	$1581.54^{+25.79}_{-28.17}$ 	\\
L4 	& 	$1706.08^{+27.08}_{-24.99}$ 	&	 $1706.56^{+26.30}_{-24.30}$ 	& 	$1696.72^{+29.27}_{-28.59}$ 	& 	& 	$1618.26^{+17.46}_{-17.85}$ 	&	 $1617.90^{+17.32}_{-17.61}$ 	& 	$1618.33^{+16.13}_{-16.60}$ 	\\
L5 	& 	$1521.41^{+25.19}_{-24.26}$ 	&	 $1482.93^{+23.12}_{-23.80}$ 	& 	$1493.11^{+23.13}_{-22.76}$ 	& 	& 	$1394.87^{+23.82}_{-24.06}$ 	&	 $1394.45^{+22.80}_{-23.40}$ 	& 	$1425.37^{+20.01}_{-20.01}$ 	\\
L6 	& 	$1561.84^{+22.67}_{-21.98}$ 	&	 $1558.38^{+21.73}_{-21.98}$ 	& 	$1564.36^{+20.10}_{-21.21}$ 	& 	& 	$1476.70^{+22.48}_{-22.51}$ 	&	 $1435.36^{+21.34}_{-21.65}$ 	& 	$1444.14^{+17.30}_{-18.91}$ 	\\
L7 	& 	$1364.02^{+34.61}_{-32.34}$ 	&	 $1332.57^{+26.97}_{-30.51}$ 	& 	$1326.71^{+33.25}_{-33.91}$ 	& 	& 	$1281.97^{+37.05}_{-33.35}$ 	&	 $1282.35^{+34.47}_{-32.08}$ 	& 	$1294.20^{+34.33}_{-31.21}$ 	\\
L8 	& 	$1220.01^{+39.70}_{-38.87}$ 	&	 $1221.46^{+40.54}_{-39.04}$ 	& 	$1229.04^{+37.71}_{-35.36}$ 	& 	& 	$1123.47^{+53.85}_{-48.80}$ 	&	 $1125.49^{+51.62}_{-46.42}$ 	& 	$1164.43^{+46.66}_{-43.99}$ 	\\
L9 	& 	$1298.89^{+31.48}_{-35.09}$ 	&	 $1349.29^{+16.20}_{-16.82}$ 	& 	$1359.59^{+17.89}_{-21.31}$ 	& 	& 	$1279.36^{+27.83}_{-27.54}$ 	&	 $1297.24^{+21.72}_{-21.88}$ 	& 	$1303.96^{+19.26}_{-19.28}$ 	\\
T0 	& 	$1333.79^{+31.91}_{-32.71}$ 	&	 $1325.20^{+28.88}_{-29.94}$ 	& 	$1328.49^{+29.06}_{-29.28}$ 	& 	& 	$1220.51^{+34.74}_{-34.67}$ 	&	 $1218.15^{+33.68}_{-32.98}$ 	& 	$1217.48^{+32.82}_{-31.47}$ 	\\
T1 	& 	$1464.51^{+26.14}_{-26.97}$ 	&	 $1461.66^{+24.90}_{-26.13}$ 	& 	$1465.75^{+24.78}_{-24.85}$ 	& 	& 	$1349.59^{+36.57}_{-39.18}$ 	&	 $1334.25^{+33.94}_{-32.75}$ 	& 	$1340.13^{+32.94}_{-31.06}$ 	\\
T2 	& 	$1169.07^{+21.85}_{-22.71}$ 	&	 $1176.50^{+22.57}_{-21.59}$ 	& 	$1171.62^{+22.00}_{-21.58}$ 	& 	& 	$1061.97^{+25.82}_{-26.21}$ 	&	 $1062.43^{+26.39}_{-28.11}$ 	& 	$1059.99^{+24.68}_{-25.65}$ 	\\
T3 	& 	$1295.39^{+36.28}_{-37.30}$ 	&	 $1297.46^{+37.22}_{-37.79}$ 	& 	$1295.48^{+35.03}_{-36.89}$ 	& 	& 	$1227.07^{+47.49}_{-48.33}$ 	&	 $1237.30^{+48.99}_{-52.22}$ 	& 	$1221.94^{+41.75}_{-43.60}$ 	\\
T4 	& 	$1124.45^{+24.47}_{-25.38}$ 	&	 $1124.28^{+23.83}_{-24.38}$ 	& 	$1120.24^{+22.77}_{-24.30}$ 	& 	& 	$1116.11^{+37.32}_{-38.24}$ 	&	 $1115.92^{+35.27}_{-36.39}$ 	& 	$1116.21^{+32.88}_{-34.58}$ 	\\
T5 	& 	$1049.15^{+26.50}_{-30.15}$ 	&	 $1047.87^{+25.79}_{-29.33}$ 	& 	$1048.70^{+24.88}_{-27.85}$ 	& 	& 	$968.86^{+34.22}_{-34.15}$	&	$967.32^{+32.82}_{-33.55}$  	&	$964.77^{+30.74}_{-33.75}$ 	\\
T6 	& 	$853.72^{+47.68}_{-52.44}$	&	$852.41^{+45.69}_{-50.57}$ 	&	$856.36^{+43.37}_{-48.99}$ 	& 	& 	$787.84^{+61.32}_{-71.06}$	&	$787.84^{+59.38}_{-65.91}$ 	&	$798.66^{+54.31}_{-63.54}$ 	\\
T7 	& 	$847.62^{+20.41}_{-21.15}$	&	$845.48^{+19.99}_{-20.98}$ 	&	$852.59^{+18.69}_{-20.49}$ 	& 	& 	$712.02^{+22.57}_{-26.18}$	&	$691.80^{+20.36}_{-26.09}$	&	$710.72^{+21.75}_{-23.84}$ 	\\
T8 	& 	$717.17^{+30.67}_{-32.00}$	&	$715.34^{+30.18}_{-31.38}$	&	$716.90^{+29.83}_{-30.65}$ 	& 	& 	$722.01^{+40.77}_{-42.74}$	&	$719.76^{+39.73}_{-41.50}$	&	$780.72^{+69.91}_{-92.76}$ 	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}




\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:log H2O entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	$-4.62^{+0.10}_{-0.10}$ 	& 	$-4.07^{+0.10}_{-0.09}$ 	& 	$-3.66^{+0.09}_{-0.08}$ 	& 	& 	$-3.54^{+0.18}_{-0.16}$ 	& 	$-3.54^{+0.17}_{-0.15}$ 	& 	$-3.05^{+0.29}_{-0.32}$ 	\\
L1 	& 	$-4.31^{+0.10}_{-0.10}$ 	& 	$-4.30^{+0.09}_{-0.09}$ 	& 	$-3.86^{+0.07}_{-0.09}$ 	& 	& 	$-3.52^{+0.33}_{-0.23}$ 	& 	$-3.52^{+0.36}_{-0.23}$ 	& 	$-3.04^{+0.38}_{-0.30}$ 	\\
L2 	& 	$-4.01^{+0.36}_{-0.67}$ 	& 	$-3.85^{+0.10}_{-0.10}$ 	& 	$-3.25^{+0.22}_{-0.18}$ 	& 	& 	$-3.35^{+0.32}_{-0.22}$ 	& 	$-3.35^{+0.22}_{-0.23}$ 	& 	$-2.55^{+0.41}_{-0.50}$ 	\\
L3 	& 	$-3.40^{+0.11}_{-0.11}$ 	& 	$-3.46^{+0.12}_{-0.12}$ 	& 	$-2.76^{+0.31}_{-0.28}$ 	& 	& 	$-3.35^{+0.12}_{-0.11}$ 	& 	$-3.36^{+0.11}_{-0.11}$ 	& 	$-3.26^{+0.14}_{-0.19}$ 	\\
L4 	& 	$-3.29^{+0.49}_{-0.48}$ 	& 	$-3.25^{+0.51}_{-0.46}$ 	& 	$-2.61^{+0.68}_{-0.51}$ 	& 	& 	$-2.73^{+0.41}_{-0.37}$ 	& 	$-2.72^{+0.41}_{-0.37}$ 	& 	$-1.89^{+0.63}_{-0.47}$ 	\\
L5 	& 	$-3.31^{+0.10}_{-0.10}$ 	& 	$-3.30^{+0.14}_{-0.13}$ 	& 	$-3.14^{+0.19}_{-0.19}$ 	& 	& 	$-3.25^{+0.14}_{-0.14}$ 	& 	$-3.25^{+0.14}_{-0.14}$ 	& 	$-2.77^{+0.22}_{-0.20}$ 	\\
L6 	& 	$-2.87^{+0.41}_{-0.37}$ 	& 	$-2.85^{+0.39}_{-0.33}$ 	& 	$-2.30^{+0.61}_{-0.50}$ 	& 	& 	$-2.92^{+0.36}_{-0.33}$ 	& 	$-2.97^{+0.34}_{-0.29}$ 	& 	$-2.25^{+0.52}_{-0.40}$ 	\\
L7 	& 	$-3.12^{+0.54}_{-0.61}$ 	& 	$-3.34^{+0.37}_{-0.40}$ 	& 	$-3.02^{+0.38}_{-0.45}$ 	& 	& 	$-3.46^{+0.40}_{-0.65}$ 	& 	$-3.43^{+0.40}_{-0.59}$ 	& 	$-3.16^{+0.57}_{-1.27}$ 	\\
L8 	& 	$-3.77^{+0.13}_{-0.13}$ 	& 	$-3.76^{+0.13}_{-0.13}$ 	& 	$-3.61^{+0.14}_{-0.13}$ 	& 	& 	$-3.90^{+0.18}_{-0.16}$ 	& 	$-3.89^{+0.18}_{-0.15}$ 	& 	$-3.53^{+0.27}_{-0.26}$ 	\\
L9 	& 	$-3.49^{+0.06}_{-0.06}$ 	& 	$-3.49^{+0.07}_{-0.08}$ 	& 	$-3.38^{+0.08}_{-0.10}$ 	& 	& 	$-3.41^{+0.09}_{-0.08}$ 	& 	$-3.46^{+0.09}_{-0.10}$ 	& 	$-3.31^{+0.08}_{-0.09}$ 	\\
T0 	& 	$-3.97^{+0.11}_{-0.35}$ 	& 	$-4.00^{+0.08}_{-0.11}$ 	& 	$-4.00^{+0.09}_{-0.15}$ 	& 	& 	$-4.08^{+0.08}_{-0.09}$ 	& 	$-4.08^{+0.07}_{-0.07}$ 	& 	$-4.09^{+0.07}_{-0.07}$ 	\\
T1 	& 	$-3.81^{+0.05}_{-0.05}$ 	& 	$-3.81^{+0.05}_{-0.05}$ 	& 	$-3.81^{+0.04}_{-0.05}$ 	& 	& 	$-3.82^{+0.06}_{-0.08}$ 	& 	$-3.84^{+0.05}_{-0.06}$ 	& 	$-3.83^{+0.05}_{-0.06}$ 	\\
T2 	& 	$-3.91^{+0.04}_{-0.04}$ 	& 	$-3.85^{+0.07}_{-0.07}$ 	& 	$-3.89^{+0.05}_{-0.06}$ 	& 	& 	$-3.93^{+0.04}_{-0.05}$ 	& 	$-3.93^{+0.04}_{-0.05}$ 	& 	$-3.93^{+0.04}_{-0.04}$ 	\\
T3 	& 	$-3.64^{+0.05}_{-0.05}$ 	& 	$-3.63^{+0.05}_{-0.06}$ 	& 	$-3.63^{+0.05}_{-0.05}$ 	& 	& 	$-3.61^{+0.05}_{-0.06}$ 	& 	$-3.59^{+0.06}_{-0.10}$ 	& 	$-3.61^{+0.05}_{-0.05}$ 	\\
T4 	& 	$-3.76^{+0.05}_{-0.05}$ 	& 	$-3.75^{+0.05}_{-0.06}$ 	& 	$-3.74^{+0.05}_{-0.05}$ 	& 	& 	$-3.50^{+0.12}_{-0.15}$ 	& 	$-3.50^{+0.12}_{-0.14}$ 	& 	$-3.49^{+0.11}_{-0.13}$ 	\\
T5 	& 	$-3.44^{+0.04}_{-0.04}$ 	& 	$-3.44^{+0.04}_{-0.04}$ 	& 	$-3.44^{+0.04}_{-0.04}$ 	& 	& 	$-3.45^{+0.05}_{-0.05}$ 	& 	$-3.45^{+0.05}_{-0.05}$ 	& 	$-3.45^{+0.05}_{-0.05}$ 	\\
T6 	& 	$-3.60^{+0.10}_{-0.10}$ 	& 	$-3.60^{+0.09}_{-0.10}$ 	& 	$-3.60^{+0.09}_{-0.10}$ 	& 	& 	$-3.63^{+0.15}_{-0.14}$ 	& 	$-3.63^{+0.14}_{-0.13}$ 	& 	$-3.61^{+0.13}_{-0.12}$ 	\\
T7 	& 	$-3.02^{+0.06}_{-0.07}$ 	& 	$-3.02^{+0.06}_{-0.06}$ 	& 	$-3.07^{+0.05}_{-0.05}$ 	& 	& 	$-3.24^{+0.05}_{-0.06}$ 	& 	$-3.26^{+0.04}_{-0.05}$ 	& 	$-3.24^{+0.05}_{-0.06}$ 	\\
T8 	& 	$-3.59^{+0.05}_{-0.06}$ 	& 	$-3.59^{+0.05}_{-0.05}$ 	& 	$-3.59^{+0.05}_{-0.05}$ 	& 	& 	$-3.58^{+0.06}_{-0.07}$ 	& 	$-3.58^{+0.06}_{-0.06}$ 	& 	$-3.46^{+0.13}_{-0.25}$ 	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}


\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:log CH4 entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L1 	& 	-	& 	-	& 	-	& 	& 	$-4.80^{+1.52}_{-0.33}$	& 	-	& 	-	\\
L2 	& 	$-5.32^{+4.23}_{-0.95}$	&	-	&	- 	& 	& 	$-4.41^{+0.40}_{-0.25}$	& 	-	& 	-	\\
L3 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L4 	& 	$-4.75^{+1.03}_{-0.5}$	&	$-4.70^{+1.09}_{-0.52}$	&	$-3.94^{+0.77}_{-0.53}$ 	& 	& 	$-4.20^{+0.46}_{-0.36}$	& 	$-4.19^{+0.45}_{-0.36}$ 	& 	$-3.32^{+0.66}_{-0.47}$ 	\\
L5 	& 	-	& 	$-4.63^{+0.46}_{-0.23}$	&	$-4.39^{+0.40}_{-0.28}$ 	& 	& 	$-4.62^{+2.17}_{-0.28}$	& 	$-4.60^{+1.91}_{-0.27}$ 	& 	$-3.90^{+0.33}_{-0.26}$ 	\\
L6 	& 	$-4.11^{+0.47}_{-0.38}$	&	$-4.07^{+0.44}_{-0.33}$	&	$-3.49^{+0.64}_{-0.50}$ 	& 	& 	$-4.06^{+0.39}_{-0.34}$	& 	$-3.94^{+0.39}_{-0.29}$ 	& 	$-3.16^{+0.56}_{-0.38}$ 	\\
L7 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L8 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L9 	& 	$-4.46^{+0.12}_{-0.11}$	&	$-4.43^{+0.12}_{-0.12}$	& 	$-4.26^{+0.13}_{-0.13}$ 	& 	& 	$-4.30^{+0.15}_{-0.12}$	& 	$-4.40^{+0.14}_{-0.14}$ 	& 	$-4.18^{+0.11}_{-0.12}$ 	\\
T0 	& 	$-5.09^{+0.17}_{-0.61}$	&	$-5.13^{+0.13}_{-0.19}$	& 	$-5.13^{+0.13}_{-0.25}$ 	& 	& 	$-5.23^{+0.12}_{-0.14}$	& 	$-5.24^{+0.11}_{-0.11}$ 	& 	$-5.24^{+0.11}_{-0.11}$ 	\\
T1 	& 	$-4.86^{+0.07}_{-0.06}$	&	$-4.84^{+0.07}_{-0.08}$	&	$-4.85^{+0.07}_{-0.07}$ 	& 	& 	$-4.84^{+0.10}_{-0.13}$	& 	$-4.89^{+0.08}_{-0.09}$ 	& 	$-4.86^{+0.08}_{-0.09}$ 	\\
T2 	& 	$-4.92^{+0.07}_{-0.06}$	&	$-4.81^{+0.12}_{-0.14}$	& 	$-4.89^{+0.08}_{-0.12}$ 	& 	& 	$-4.94^{+0.07}_{-0.07}$	& 	$-4.94^{+0.07}_{-0.07}$ 	& 	$-4.94^{+0.07}_{-0.07}$ 	\\
T3 	& 	$-4.09^{+0.07}_{-0.07}$	&	$-4.08^{+0.07}_{-0.08}$	&	$-4.08^{+0.07}_{-0.07}$ 	& 	& 	$-4.06^{+0.07}_{-0.08}$	& 	$-4.03^{+0.09}_{-0.14}$ 	& 	$-4.07^{+0.06}_{-0.06}$ 	\\
T4 	& 	$-4.37^{+0.06}_{-0.06}$	&	$-4.35^{+0.07}_{-0.09}$	&	$-4.35^{+0.06}_{-0.06}$ 	& 	& 	$-3.95^{+0.16}_{-0.19}$	& 	$-3.95^{+0.16}_{-0.18}$ 	& 	$-3.94^{+0.15}_{-0.17}$ 	\\
T5 	& 	$-3.73^{+0.06}_{-0.06}$	&	$-3.73^{+0.06}_{-0.06}$	&	$-3.73^{+0.05}_{-0.06}$ 	& 	& 	$-3.76^{+0.07}_{-0.07}$	& 	$-3.76^{+0.07}_{-0.07}$ 	& 	$-3.76^{+0.07}_{-0.07}$ 	\\
T6 	& 	$-3.75^{+0.15}_{-0.14}$	&	$-3.76^{+0.14}_{-0.13}$	& 	$-3.75^{+0.14}_{-0.13}$ 	& 	& 	$-3.80^{+0.27}_{-0.19}$	& 	$-3.79^{+0.25}_{-0.18}$ 	& 	$-3.77^{+0.23}_{-0.16}$ 	\\
T7 	& 	$-3.26^{+0.08}_{-0.09}$	&	$-3.26^{+0.07}_{-0.08}$	& 	$-3.39^{+0.08}_{-0.08}$ 	& 	& 	$-3.73^{+0.08}_{-0.11}$	& 	$-3.79^{+0.06}_{-0.08}$ 	& 	$-3.73^{+0.08}_{-0.10}$ 	\\
T8 	& 	$-3.94^{+0.06}_{-0.07}$	&	$-3.94^{+0.05}_{-0.06}$	&	$-3.94^{+0.05}_{-0.06}$ 	& 	& 	$-3.94^{+0.06}_{-0.08}$	& 	$-3.94^{+0.06}_{-0.08}$ 	& 	$-3.73^{+0.22}_{-0.37}$ 	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}



\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:log NH3 entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L1 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L2 	& 	-	&	-	&	- 	& 	& 	-	& 	-	& 	-	\\
L3 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L4 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
L5 	& 	-	& 	-	&	-	& 	& 	-	&	-	& 	-	\\
L6 	& 	$-4.57^{+0.65}_{-0.43}$ 	& 	$-4.54^{+0.62}_{-0.40}$ 	& 	$-4.04^{+0.92}_{-0.61}$ 	& 	& 	$-4.06^{+0.39}_{-0.34}$	& 	-	& 	-	\\
L7 	& 	$-4.35^{+0.58}_{-0.58}$ 	& 	$-4.45^{+0.46}_{-0.41}$ 	& 	$-3.99^{+0.43}_{-0.40}$ 	& 	& 	$-4.68^{+0.46}_{-0.65}$	& 	$-4.64^{+0.45}_{-0.59}$	& 	$-4.39^{+0.61}_{-1.23}$ 	\\
L8 	& 	$-4.45^{+0.15}_{-0.15}$ 	& 	$-4.45^{+0.15}_{-0.14}$ 	& 	$-4.24^{+0.18}_{-0.15}$ 	& 	& 	$-4.57^{+0.20}_{-0.17}$	& 	$-4.57^{+0.19}_{-0.16}$	& 	$-4.13^{+0.33}_{-0.32}$ 	\\
L9 	& 	$-5.05^{+3.06}_{-0.21}$	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T0 	& 	$-5.63^{+1.11}_{-0.70}$	&	$-5.76^{+1.32}_{-0.35}$	& 	$-5.77^{+1.79}_{-0.47}$ 	& 	& 	$-6.09^{+3.08}_{-0.46}$	& 	$-6.13^{+3.12}_{-0.43}$	& 	$-6.22^{+3.22}_{-0.47}$ 	\\
T1 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
T2 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T3 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
T4 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
T5 	& 	$-5.39^{+0.40}_{-0.18}$	&	$-5.39^{+0.37}_{-0.18}$	&	$-5.39^{+0.33}_{-0.17}$ 	& 	& 	$-5.65^{+3.17}_{-0.31}$	& 	$-5.65^{+3.21}_{-0.31}$	& 	$-5.62^{+2.82}_{-0.28}$ 	\\
T6 	& 	$-4.97^{+0.21}_{-0.18}$	&	$-4.97^{+0.20}_{-0.18}$	& 	$-4.97^{+0.20}_{-0.18}$ 	& 	& 	$-5.02^{+0.34}_{-0.24}$	& 	$-5.01^{+0.32}_{-0.23}$	& 	$-5.00^{+0.31}_{-0.22}$ 	\\
T7 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T8 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}


\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:log CO2 entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	-	& 	-	& 	$-2.90^{+0.14}_{-0.13}$ 	& 	& 	-	& 	-	& 	-	\\
L1 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L2 	& 	-	&	-	&	- 	& 	& 	- 	& 	- 	& 	- 	\\
L3 	& 	-	& 	-	& 	$-3.29^{+5.02}_{-0.46}$ 	& 	& 	-	& 	-	& 	-	\\
L4 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
L5 	& 	-	& 	-	&	-	& 	& 	-	&	-	& 	-	\\
L6 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L7 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L8 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L9 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T0 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T1 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
T2 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T3 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
T4 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
T5 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
T6 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T7 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T8 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}

\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:log CO entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	-	& 	-	& 	$-2.29^{+0.29}_{-0.24}$ 	& 	& 	-	& 	-	& 	-	\\
L1 	& 	-	& 	-	& 	$-3.22^{+0.26}_{-0.22}$ 	& 	& 	-	& 	-	& 	-	\\
L2 	& 	-	&	$-3.22^{+0.27}_{-0.23}$	&	$-2.80^{+0.26}_{-0.25}$ 	& 	& 	$-4.08^{+4.33}_{-0.69}$	& 	$-3.92^{+3.79}_{-0.73}$	& 	$-2.89^{+4.33}_{-0.59}$	\\
L3 	& 	$-2.95^{+0.32}_{-0.28}$	& 	$-3.00^{+0.26}_{-0.24}$	& 	$-2.30^{+0.35}_{-0.33}$ 	& 	& 	$-2.77^{+0.25}_{-0.22}$	& 	$-2.77^{+0.24}_{-0.22}$	& 	$-2.75^{+0.23}_{-0.21}$ 	\\
L4 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
L5 	& 	$-2.95^{+0.18}_{-0.18}$	& 	$-3.12^{+0.20}_{-0.20}$	&	$-3.02^{+0.20}_{-0.20}$ 	& 	& 	$-2.91^{+0.19}_{-0.18}$	&	$-2.91^{+0.18}_{-0.18}$	& 	$-2.68^{+0.21}_{-0.22}$ 	\\
L6 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L7 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L8 	& 	$-2.68^{+0.18}_{-0.18}$	& 	$-2.67^{+0.19}_{-0.18}$	& 	$-2.60^{+0.17}_{-0.16}$ 	& 	& 	$-2.77^{+0.23}_{-0.19}$	& 	$-2.76^{+0.23}_{-0.19}$	& 	$-2.54^{+0.23}_{-0.27}$ 	\\
L9 	& 	$-3.42^{+0.41}_{-0.23}$	&	$-3.60^{+0.60}_{-0.26}$	& 	$-3.54^{+0.76}_{-0.25}$ 	& 	& 	$-4.02^{+4.98}_{-0.65}$	& 	$-3.99^{+4.55}_{-0.52}$	& 	$-3.85^{+4.66}_{-0.46}$ 	\\
T0 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T1 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
T2 	& 	$-3.69^{+0.29}_{-0.25}$	&	$-3.66^{+0.23}_{-0.19}$	& 	$-3.69^{+0.24}_{-0.21}$ 	& 	& 	$-3.80^{+0.26}_{-0.24}$	& 	$-3.80^{+0.26}_{-0.23}$	& 	$-3.81^{+0.25}_{-0.22}$ 	\\
T3 	& 	$-2.85^{+0.21}_{-0.19}$	&	$-2.83^{+0.21}_{-0.18}$	&	$-2.84^{+0.20}_{-0.18}$ 	& 	& 	$-2.87^{+0.24}_{-0.20}$	& 	$-2.82^{+0.23}_{-0.21}$	& 	$-2.84^{+0.21}_{-0.19}$ 	\\
T4 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
T5 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
T6 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T7 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T8 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}



\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:log H2S entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	$-4.14^{+0.15}_{-0.13}$	& 	$-3.47^{+0.13}_{-0.11}$ 	& 	-	& 	& 	$-3.24^{+1.25}_{-0.21}$	& 	$-3.25^{+1.84}_{-0.22}$	& 	$-3.28^{+5.37}_{-0.51}$ 	\\
L1 	& 	-	& 	-	& 	$-3.37^{+0.11}_{-0.12}$ 	& 	& 	-	& 	-	& 	-	\\
L2 	& 	$-3.63^{+0.40}_{-0.69}$	&	$-3.34^{+0.12}_{-0.11}$	&	$-2.69^{+0.25}_{-0.22}$ 	& 	& 	$-3.02^{+0.34}_{-0.23}$	& 	$-2.99^{+0.24}_{-0.20}$	& 	$-2.11^{+0.46}_{-0.42}$ 	\\
L3 	& 	$-3.67^{+5.02}_{-0.38}$	& 	$-3.35^{+0.19}_{-0.15}$	& 	$-2.59^{+1.48}_{-0.35}$ 	& 	& 	$-3.09^{+0.14}_{-0.12}$	& 	$-3.09^{+0.14}_{-0.12}$	& 	$-3.06^{+0.18}_{-0.15}$ 	\\
L4 	& 	-	&	-	&	$-3.70^{+4.98}_{-1.19}$ 	& 	& 	-	& 	-	& 	-	\\
L5 	& 	-	& 	$-3.20^{+0.21}_{-0.16}$	&	$-3.04^{+0.25}_{-0.22}$	& 	& 	$-3.06^{+0.24}_{-0.19}$	&	$-3.06^{+0.24}_{-0.18}$	& 	$-2.59^{+0.27}_{-0.23}$	\\
L6 	& 	-	& 	-	& 	-	& 	& 	-	& 	$-2.87^{+0.41}_{-0.30}$	& 	$-2.07^{+0.61}_{-0.39}$ 	\\
L7 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L8 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L9 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T0 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T1 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
T2 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T3 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
T4 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
T5 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
T6 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T7 	& 	-	&	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T8 	& 	-	&	-	&	-	& 	& 	-	& 	-	& 	-	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}


\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:log K entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	$-6.71^{+0.18}_{-0.17}$ 	& 	$-6.42^{+0.15}_{-0.13}$ 	& 	$-7.36^{+0.16}_{-0.15}$ 	& 	& 	-	& 	-	& 	-	\\
L1 	& 	$-6.37^{+0.15}_{-0.15}$ 	& 	$-6.36^{+0.15}_{-0.14}$ 	& 	$-6.38^{+0.12}_{-0.10}$ 	& 	& 	$-6.30^{+1.52}_{-0.62}$	& 	$-5.73^{+0.39}_{-0.36}$	& 	$-6.20^{+1.80}_{-0.73}$ 	\\
L2 	& 	$-6.37^{+0.48}_{-0.77}$ 	& 	$-6.61^{+0.18}_{-0.17}$ 	& 	$-6.52^{+0.25}_{-0.27}$ 	& 	& 	$-5.00^{+0.36}_{-0.29}$	& 	$-5.19^{+0.46}_{-0.36}$	& 	$-4.68^{+0.65}_{-0.86}$ 	\\
L3 	& 	$-6.16^{+0.18}_{-0.18}$ 	& 	$-6.06^{+0.15}_{-0.15}$ 	& 	$-5.72^{+0.49}_{-0.37}$ 	& 	& 	-	& 	-	& 	$-7.10^{+2.88}_{-1.16}$ 	\\
L4 	& 	$-5.54^{+0.51}_{-0.53}$ 	& 	$-5.51^{+0.52}_{-0.52}$ 	& 	$-4.89^{+0.69}_{-0.56}$ 	& 	& 	$-4.70^{+0.58}_{-0.60}$	& 	$-4.66^{+0.54}_{-0.58}$	& 	$-3.95^{+0.76}_{-0.63}$ 	\\
L5 	& 	$-6.37^{+0.15}_{-0.15}$ 	& 	$-6.06^{+0.18}_{-0.16}$ 	& 	$-5.97^{+0.21}_{-0.22}$ 	& 	& 	-	&	-	& 	-	\\
L6 	& 	$-5.27^{+0.45}_{-0.46}$ 	& 	$-5.28^{+0.42}_{-0.43}$ 	& 	$-4.75^{+0.61}_{-0.56}$ 	& 	& 	$-4.87^{+2.54}_{-0.56}$	& 	-	& 	-	\\
L7 	& 	$-5.93^{+0.72}_{-0.88}$ 	& 	$-6.48^{+0.48}_{-0.56}$ 	& 	$-6.71^{+2.00}_{-0.99}$ 	& 	& 	$-5.13^{+0.51}_{-0.65}$	& 	$-5.21^{+0.66}_{-0.64}$	& 	$-5.59^{+2.89}_{-1.55}$ 	\\
L8 	& 	$-7.92^{+0.27}_{-0.26}$ 	& 	$-7.89^{+0.27}_{-0.27}$ 	& 	$-7.89^{+0.34}_{-0.27}$ 	& 	& 	-	& 	-	& 	-	\\
L9 	& 	$-7.34^{+0.17}_{-0.18}$ 	& 	$-6.88^{+0.11}_{-0.10}$ 	& 	$-6.88^{+0.11}_{-0.12}$ 	& 	& 	$-6.32^{+1.15}_{-0.35}$	& 	-	& 	-	\\
T0 	& 	$-7.29^{+0.16}_{-0.17}$ 	& 	$-7.32^{+0.14}_{-0.15}$ 	& 	$-7.31^{+0.15}_{-0.15}$ 	& 	& 	-	& 	-	& 	-	\\
T1 	& 	$-6.46^{+0.10}_{-0.10}$ 	& 	$-6.46^{+0.10}_{-0.10}$ 	& 	$-6.44^{+0.10}_{-0.09}$ 	& 	& 	$-6.47^{+0.92}_{-0.43}$	& 	$-7.27^{+2.17}_{-0.60}$	& 	$-6.69^{+1.18}_{-0.46}$ 	\\
T2 	& 	$-6.78^{+0.08}_{-0.08}$ 	& 	$-6.79^{+0.07}_{-0.07}$ 	& 	$-6.79^{+0.07}_{-0.07}$ 	& 	& 	$-6.83^{+1.93}_{-0.49}$	& 	$-6.87^{+1.92}_{-0.51}$	& 	$-6.90^{+1.89}_{-0.51}$ 	\\
T3 	& 	$-7.04^{+0.11}_{-0.11}$ 	& 	$-7.02^{+0.11}_{-0.12}$ 	& 	$-7.04^{+0.11}_{-0.11}$ 	& 	& 	-	& 	-	& 	-	\\
T4 	& 	$-6.51^{+0.08}_{-0.08}$ 	& 	$-6.52^{+0.08}_{-0.08}$ 	& 	$-6.49^{+0.08}_{-0.07}$ 	& 	& 	-	& 	-	& 	-	\\
T5 	& 	$-6.87^{+0.05}_{-0.06}$ 	& 	$-6.87^{+0.05}_{-0.06}$ 	& 	$-6.87^{+0.05}_{-0.05}$ 	& 	& 	-	& 	-	& 	-	\\
T6 	& 	$-7.17^{+0.12}_{-0.13}$ 	& 	$-7.16^{+0.11}_{-0.12}$ 	& 	$-7.15^{+0.11}_{-0.12}$ 	& 	& 	-	& 	-	& 	-	\\
T7 	& 	$-6.68^{+0.08}_{-0.08}$ 	& 	$-6.68^{+0.08}_{-0.08}$ 	& 	$-6.86^{+0.12}_{-0.10}$ 	& 	& 	-	& 	$-5.99^{+3.27}_{-0.42}$	& 	-	\\
T8 	& 	$-7.07^{+0.11}_{-0.11}$ 	& 	$-7.07^{+0.11}_{-0.11}$ 	& 	$-7.05^{+0.11}_{-0.11}$ 	& 	& 	-	& 	-	& 	-	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}





\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:log CrH entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	$-8.94^{+0.24}_{-0.21}$	& 	$-8.46^{+0.21}_{-0.19}$	& 	$-8.08^{+0.13}_{-0.13}$ 	& 	& 	$-7.64^{+0.97}_{-0.43}$	& 	$-7.61^{+0.75}_{-0.40}$	& 	$-7.58^{+2.27}_{-0.69}$ 	\\
L1 	& 	$-9.00^{+0.35}_{-0.27}$	& 	$-8.99^{+0.32}_{-0.26}$	& 	$-8.63^{+0.23}_{-0.24}$ 	& 	& 	$-8.52^{+2.05}_{-0.99}$	& 	-	& 	-	\\
L2 	& 	$-8.25^{+0.43}_{-0.65}$	& 	$-8.14^{+0.16}_{-0.16}$	& 	$-7.36^{+0.25}_{-0.22}$ 	& 	& 	-	& 	$-7.41^{+2.18}_{-0.56}$	& 	$-6.62^{+2.17}_{-0.62}$ 	\\
L3 	& 	$-8.10^{+0.28}_{-0.24}$	& 	$-8.36^{+0.31}_{-0.27}$	& 	$-7.37^{+0.32}_{-0.28}$ 	& 	& 	-	& 	-	& 	-	\\
L4 	& 	$-7.44^{+0.51}_{-0.52}$	& 	$-7.40^{+0.53}_{-0.50}$	& 	$-6.78^{+0.70}_{-0.54}$ 	& 	& 	$-6.70^{+1.91}_{-0.68}$	& 	$-6.69^{+1.66}_{-0.67}$	& 	$-6.07^{+2.29}_{-0.85}$ 	\\
L5 	& 	-	& 	-	& 	-	& 	& 	-	&	-	& 	-	\\
L6 	& 	$-7.29^{+0.47}_{-0.44}$	& 	$-7.31^{+0.43}_{-0.42}$	& 	$-6.73^{+0.63}_{-0.54}$ 	& 	& 	-	& 	-	& 	-	\\
L7 	& 	$-7.68^{+0.68}_{-0.73}$	& 	$-7.74^{+0.38}_{-0.43}$	& 	$-7.46^{+0.41}_{-0.52}$ 	& 	& 	-	& 	-	& 	-	\\
L8 	& 	$-8.83^{+0.24}_{-0.21}$	& 	$-8.83^{+0.23}_{-0.21}$	& 	$-8.65^{+0.23}_{-0.20}$ 	& 	& 	-	& 	-	& 	-	\\
L9 	& 	$-8.64^{+0.14}_{-0.13}$	& 	$-8.59^{+0.13}_{-0.13}$	& 	$-8.46^{+0.13}_{-0.14}$ 	& 	& 	-	& 	-	& 	-	\\
T0 	& 	$-9.01^{+0.18}_{-0.32}$	& 	$-9.06^{+0.15}_{-0.14}$	& 	$-9.06^{+0.16}_{-0.18}$	& 	& 	-	& 	-	& 	-	\\
T1 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T2 	& 	$-9.47^{+0.21}_{-0.17}$	& 	$-9.40^{+0.20}_{-0.16}$	& 	-	& 	& 	-	& 	-	& 	-	\\
T3 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T4 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T5 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T6 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T7 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T8 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	$-7.53^{+1.84}_{-0.53}$	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}




\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:log FeH entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	$-9.18^{+0.52}_{-0.32}$ 	& 	$-8.74^{+0.40}_{-0.26}$ 	& 	-	& 	& 	$-6.99^{+0.28}_{-0.19}$	& 	$-7.02^{+0.32}_{-0.20}$	& 	-	\\
L1 	& 	$-8.68^{+0.27}_{-0.23}$ 	& 	$-8.68^{+0.25}_{-0.21}$ 	& 	$-8.39^{+0.19}_{-0.16}$ 	& 	& 	$-7.81^{+2.20}_{-0.53}$ 	& 	-	& 	$-7.06^{+0.48}_{-0.36}$ 	\\
L2 	& 	$-8.44^{+0.52}_{-0.78}$ 	& 	$-8.58^{+0.28}_{-0.25}$ 	& 	$-8.78^{+1.32}_{-0.46}$ 	& 	& 	-	& 	-	& 	-	\\
L3 	& 	$-7.84^{+0.21}_{-0.20}$ 	& 	$-7.76^{+0.17}_{-0.16}$ 	& 	$-7.42^{+0.47}_{-0.39}$ 	& 	& 	$-6.83^{+0.13}_{-0.12}$	& 	$-6.84^{+0.12}_{-0.12}$	& 	$-6.89^{+0.18}_{-0.15}$	\\
L4 	& 	$-7.62^{+0.49}_{-0.52}$ 	& 	$-7.58^{+0.51}_{-0.50}$ 	& 	$-6.92^{+0.69}_{-0.56}$ 	& 	& 	-	& 	-	& 	-	\\
L5 	& 	$-8.07^{+0.16}_{-0.15}$ 	& 	$-7.99^{+0.19}_{-0.18}$ 	& 	$-7.83^{+0.23}_{-0.22}$ 	& 	& 	$-7.06^{+0.20}_{-0.18}$	&	$-7.07^{+0.20}_{-0.18}$	& 	$-6.64^{+0.25}_{-0.23}$ 	\\
L6 	& 	$-7.51^{+0.48}_{-0.46}$ 	& 	$-7.50^{+0.45}_{-0.43}$ 	& 	$-7.00^{+0.62}_{-0.58}$ 	& 	& 	$-7.68^{+2.73}_{-0.93}$	& 	$-6.43^{+0.35}_{-0.30}$	& 	$-5.71^{+0.53}_{-0.42}$ 	\\
L7 	& 	$-9.37^{+1.55}_{-1.26}$	& 	-	& 	-	& 	& 	-	& 	-	& 	$-8.05^{+1.51}_{-0.96}$ 	\\
L8 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L9 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T0 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T1 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T2 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T3 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T4 	& 	$-9.44^{+0.20}_{-0.17}$ 	& 	$-9.42^{+0.19}_{-0.16}$	& 	$-9.42^{+0.18}_{-0.16}$ 	& 	& 	$-7.27^{+0.20}_{-0.20}$	& 	$-7.27^{+0.19}_{-0.18}$ 	& 	$-7.26^{+0.17}_{-0.17}$ 	\\
T5 	& 	$-9.60^{+0.12}_{-0.11}$ 	& 	$-9.60^{+0.12}_{-0.11}$	& 	$-9.62^{+0.14}_{-0.11}$ 	& 	& 	$-7.96^{+0.18}_{-0.15}$	& 	$-7.96^{+0.17}_{-0.15}$	& 	$-7.96^{+0.15}_{-0.13}$ 	\\
T6 	& 	$-10.25^{+0.76}_{-0.33}$	 &	 $-10.24^{+0.72}_{-0.32}$	 	& $-10.25^{+0.69}_{-0.31}$ 	& 	& 	-	& 	-	& 	-	\\
T7 	& 	$-10.12^{+0.96}_{-0.38}$	 &	 $-10.11^{+0.92}_{-0.38}$	 &	-	& 	& 	$-7.79^{+0.25}_{-0.19}$	& 	$-8.69^{+2.13}_{-0.90}$	& 	$-7.79^{+0.24}_{-0.17}$ 	\\
T8 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}




\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:log CaH entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L1 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L2 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L3 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L4 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L5 	& 	-	& 	-	& 	-	& 	& 	-	&	-	& 	-	\\
L6 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L7 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L8 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L9 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T0 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T1 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T2 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T3 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T4 	& 	$3.52^{+0.12}_{-0.12}$	& 	-	& 	$-3.59^{+4.94}_{-0.91}$ 	& 	& 	-	& 	-	& 	-	\\
T5 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T6 	& 	-	 &	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T7 	& 	-	 &	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T8 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}


\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:log TiH entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L1 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L2 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L3 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L4 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L5 	& 	-	& 	-	& 	-	& 	& 	-	&	-	& 	-	\\
L6 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L7 	& 	-	& 	-	& 	$-10.54^{+0.88}_{-0.91}$ 	& 	& 	-	& 	-	& 	-	\\
L8 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
L9 	& 	-	& 	-	& 	$-10.61^{+0.79}_{-0.61}$ 	& 	& 	-	& 	-	& 	-	\\
T0 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T1 	& 	-	& 	-	& 	-	& 	& 	$-8.60^{+1.83}_{-0.45}$	& 	-	& 	$-8.93^{+1.78}_{-0.58}$ 	\\
T2 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T3 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T4 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
T5 	& 	$-10.50^{+0.55}_{-0.28}$	& 	$-10.50^{+0.52}_{-0.28}$	& 	$-10.54^{+0.57}_{-0.30}$ 	& 	& 	-	& 	-	& 	-	\\
T6 	& 	$-10.24^{+0.52}_{-0.32}$	 &	$-10.24^{+0.51}_{-0.31}$ 	& 	$-10.24^{+0.48}_{-0.31}$ 	& 	& 	-	& 	-	& 	-	\\
T7 	& 	$-10.09^{+0.74}_{-0.37}$	 &	$-10.08^{+0.69}_{-0.35}$ 	& 	-	& 	& 	-	& 	-	& 	-	\\
T8 	& 	-	& 	-	& 	-	& 	& 	-	& 	-	& 	-	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}





\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:cloud top pressure entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	- 	& 	$0.52^{+0.27}_{-0.28}$ 	& 	$0.55^{+0.27}_{-0.26}$ 	& 	& 	- 	& 	$0.51^{+0.26}_{-0.28}	$ 	& $0.52^{+0.25}_{-0.26}$ 	\\
L1 	& 	- 	& 	$0.54^{+0.27}_{-0.27}$ 	& 	$0.53^{+0.27}_{-0.26}$ 	& 	& 	- 	& 	$0.54^{+0.27}_{-0.25}	$ 	& $0.54^{+0.25}_{-0.25}$ 	\\
L2 	& 	- 	& 	$0.54^{+0.27}_{-0.26}$ 	& 	$0.56^{+0.27}_{-0.25}$ 	& 	& 	- 	& 	$0.52^{+0.25}_{-0.26}	$ 	& $0.53^{+0.25}_{-0.25}$ 	\\
L3 	& 	- 	& 	$0.62^{+0.31}_{-0.23}$ 	& 	$0.55^{+0.28}_{-0.26}$ 	& 	& 	- 	& 	$0.65^{+0.32}_{-0.21}	$ 	& $0.62^{+0.30}_{-0.23}$ 	\\
L4 	& 	- 	& 	$0.52^{+0.26}_{-0.27}$ 	& 	$0.53^{+0.25}_{-0.26}$ 	& 	& 	- 	& 	$0.50^{+0.23}_{-0.26}	$ 	& $0.51^{+0.23}_{-0.25}$ 	\\
L5 	& 	- 	& 	$0.54^{+0.27}_{-0.26}$ 	& 	$0.53^{+0.26}_{-0.26}$ 	& 	& 	- 	& 	$0.55^{+0.27}_{-0.26}	$ 	& $0.54^{+0.26}_{-0.25}$ 	\\
L6 	& 	- 	& 	$0.57^{+0.25}_{-0.25}$ 	& 	$0.57^{+0.25}_{-0.24}$ 	& 	& 	- 	& 	$0.54^{+0.25}_{-0.25}	$ 	& $0.54^{+0.24}_{-0.24}$ 	\\
L7 	& 	- 	& 	$0.53^{+0.26}_{-0.25}$ 	& 	$0.54^{+0.25}_{-0.25}$ 	& 	& 	- 	& 	$0.52^{+0.25}_{-0.26}	$ 	& $0.51^{+0.24}_{-0.25}$ 	\\
L8 	& 	- 	& 	$0.59^{+0.27}_{-0.24}$ 	& 	$0.58^{+0.26}_{-0.23}$ 	& 	& 	- 	& 	$0.59^{+0.27}_{-0.23}	$ 	& $0.60^{+0.25}_{-0.22}$ 	\\
L9 	& 	- 	& 	$0.69^{+0.21}_{-0.17}$ 	& 	$0.66^{+0.22}_{-0.18}$ 	& 	& 	- 	& 	$0.67^{+0.22}_{-0.18}	$ 	& $0.65^{+0.21}_{-0.18}$ 	\\
T0 	& 	- 	& 	$0.60^{+0.26}_{-0.23}$ 	& 	$0.61^{+0.26}_{-0.22}$ 	& 	& 	- 	& 	$0.60^{+0.25}_{-0.22}	$ 	& $0.60^{+0.25}_{-0.22}$ 	\\
T1 	& 	- 	& 	$0.65^{+0.25}_{-0.20}$ 	& 	$0.65^{+0.24}_{-0.20}$ 	& 	& 	- 	& 	$0.64^{+0.25}_{-0.20}	$ 	& $0.64^{+0.24}_{-0.20}$ 	\\
T2 	& 	- 	& 	$0.61^{+0.26}_{-0.21}$ 	& 	$0.59^{+0.26}_{-0.22}$ 	& 	& 	- 	& 	$0.60^{+0.26}_{-0.22}	$ 	& $0.60^{+0.25}_{-0.22}$ 	\\
T3 	& 	- 	& 	$0.58^{+0.28}_{-0.24}$ 	& 	$0.58^{+0.27}_{-0.24}$ 	& 	& 	- 	& 	$0.58^{+0.27}_{-0.24}	$ 	& $0.57^{+0.26}_{-0.25}$ 	\\
T4 	& 	- 	& 	$0.55^{+0.27}_{-0.26}$ 	& 	$0.54^{+0.26}_{-0.25}$ 	& 	& 	- 	& 	$0.56^{+0.27}_{-0.25}	$ 	& $0.55^{+0.26}_{-0.25}$ 	\\
T5 	& 	- 	& 	$0.59^{+0.27}_{-0.24}$ 	& 	$0.60^{+0.27}_{-0.24}$ 	& 	& 	- 	& 	$0.59^{+0.26}_{-0.24}	$ 	& $0.59^{+0.25}_{-0.23}$ 	\\
T6 	& 	- 	& 	$0.66^{+0.25}_{-0.20}$ 	& 	$0.66^{+0.25}_{-0.20}$ 	& 	& 	- 	& 	$0.65^{+0.25}_{-0.20}	$ 	& $0.64^{+0.24}_{-0.20}$ 	\\
T7 	& 	- 	& 	$0.61^{+0.26}_{-0.23}$ 	& 	$0.60^{+0.24}_{-0.21}$ 	& 	& 	- 	& 	$0.58^{+0.26}_{-0.24}	$ 	& $0.58^{+0.25}_{-0.24}$ 	\\
T8 	& 	- 	& 	$0.58^{+0.28}_{-0.25}$ 	& 	$0.58^{+0.27}_{-0.25}$ 	& 	& 	- 	& 	$0.58^{+0.28}_{-0.25}	$ 	& $0.58^{+0.26}_{-0.24}$ 	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}




\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:cloud bottom pressure entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	- 	& 	$3.79^{+0.61}_{-1.06}$ 	& 	$0.80^{+0.76}_{-11.89}$ 	& 	& 	- 	& 	$1.80^{+1.73}_{-9.21}$ 	& 	$1.32^{+1.25}_{-11.99}$ 	\\
L1 	& 	- 	& 	$2.03^{+1.93}_{-8.01}$ 	& 	$5.41^{+1.11}_{-2.03}$ 	& 	& 	- 	& 	$2.25^{+2.11}_{-6.56}$ 	& 	$1.75^{+1.66}_{-10.20}$ 	\\
L2 	& 	- 	& 	$5.15^{+1.22}_{-1.60}$ 	& 	$1.32^{+1.27}_{-15.49}$ 	& 	& 	- 	& 	$2.83^{+2.70}_{-6.17}$ 	& 	$4.01^{+3.86}_{-8.10}$ 	\\
L3 	& 	- 	& 	$4.78^{+1.20}_{-1.88}$ 	& 	$1.80^{+1.74}_{-15.70}$ 	& 	& 	- 	& 	$1.35^{+1.29}_{-15.15}$	 &	 $1.29^{+1.23}_{-13.68}$ 	\\
L4 	& 	- 	& 	$1.61^{+1.54}_{-11.95}$	 &	 $1.61^{+1.53}_{-11.71}$ 	& 	& 	- 	& 	$1.32^{+1.22}_{-9.47}$ 	& 	$1.34^{+1.24}_{-9.08}$ 	\\
L5 	& 	- 	& 	$5.29^{+1.04}_{-1.50}$ 	& 	$7.06^{+1.60}_{-2.35}$ 	& 	& 	- 	& 	$2.17^{+2.11}_{-13.62}$	 &	 $1.43^{+1.37}_{-15.69}$ 	\\
L6 	& 	- 	& 	$2.07^{+1.92}_{-6.46}$ 	& 	$2.32^{+2.19}_{-8.13}$ 	& 	& 	- 	& 	$1.66^{+1.59}_{-11.47}$	 &	 $1.58^{+1.50}_{-11.06}$ 	\\
L7 	& 	- 	& 	$2.49^{+1.25}_{-1.67}$ 	& 	$5.55^{+3.41}_{-4.72}$ 	& 	& 	- 	& 	$1.29^{+1.19}_{-7.06}$ 	& 	$1.41^{+1.30}_{-5.96}$ 	\\
L8 	& 	- 	& 	$2.07^{+2.01}_{-18.02}$	 &	 $0.93^{+0.88}_{-13.52}$ 	& 	& 	- 	& 	$2.25^{+2.18}_{-16.64}$	 &	 $1.09^{+1.03}_{-13.58}$ 	\\
L9 	& 	- 	& 	$7.37^{+1.70}_{-2.30}$ 	& 	$12.12^{+3.15}_{-4.08}$ 	& 	& 	- 	& 	$6.79^{+1.54}_{-2.19}$ 	& 	$13.49^{+2.83}_{-4.22}$ 	\\
T0 	& 	- 	& 	$3.50^{+3.41}_{-9.50}$ 	& 	$2.15^{+2.07}_{-11.41}$ 	& 	& 	- 	& 	$1.66^{+1.59}_{-12.29}$	 &	 $1.66^{+1.58}_{-12.16}$ 	\\
T1 	& 	- 	& 	$3.77^{+3.68}_{-9.20}$ 	& 	$2.66^{+2.58}_{-12.97}$ 	& 	& 	- 	& 	$2.55^{+2.47}_{-11.16}$	 &	 $1.78^{+1.71}_{-12.95}$ 	\\
T2 	& 	- 	& 	$3.55^{+2.79}_{-1.70}$ 	& 	$3.42^{+3.26}_{-6.08}$ 	& 	& 	- 	& 	$2.08^{+2.01}_{-11.54}$	 &	 $1.95^{+1.87}_{-12.24}$ 	\\
T3 	& 	- 	& 	$3.17^{+3.11}_{-25.97}$	 &	 $1.95^{+1.90}_{-25.98}$ 	& 	& 	- 	& 	$5.80^{+5.72}_{-22.12}$	 &	 $1.23^{+1.18}_{-16.72}$ 	\\
T4 	& 	- 	& 	$2.98^{+2.89}_{-10.56}$	 &	 $1.92^{+1.85}_{-13.37}$ 	& 	& 	- 	& 	$1.65^{+1.59}_{-14.88}$	 &	 $1.60^{+1.53}_{-14.18}$ 	\\
T5 	& 	- 	& 	$1.32^{+1.28}_{-18.18}$	 &	 $2.27^{+2.21}_{-15.30}$ 	& 	& 	- 	& 	$1.22^{+1.17}_{-16.04}$	 &	 $1.28^{+1.22}_{-15.44}$ 	\\
T6 	& 	- 	& 	$1.19^{+1.14}_{-16.21}$	 &	 $1.22^{+1.17}_{-15.52}$ 	& 	& 	- 	& 	$1.18^{+1.13}_{-13.99}$	 &	 $1.23^{+1.17}_{-14.12}$ 	\\
T7 	& 	- 	& 	$1.38^{+1.33}_{-17.13}$	 &	 $2.50^{+0.78}_{-0.78}$ 	& 	& 	- 	& 	$1.80^{+1.73}_{-13.92}$	 &	 $1.68^{+1.62}_{-13.79}$ 	\\
T8 	& 	- 	& 	$1.60^{+1.55}_{-15.51}$	 &	 $1.55^{+1.50}_{-14.98}$ 	& 	& 	- 	& 	$1.86^{+1.80}_{-14.10}$	 &	 $1.70^{+1.64}_{-11.76}$ 	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}




\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:cloud tau entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	- 	& 	$2.36^{+1.01}_{-2.93}$ 	& 	$3.21^{+1.69}_{-3.57}$ 	& 	& 	- 	& 	$3.20^{+1.66}_{-3.40}$ 	& 	$3.22^{+1.63}_{-3.20}$ 	\\
L1 	& 	- 	& 	$3.12^{+1.62}_{-3.51}$ 	& 	$2.78^{+1.29}_{-2.94}$ 	& 	& 	- 	& 	$3.13^{+1.58}_{-3.36}$ 	& 	$3.21^{+1.63}_{-3.20}$ 	\\
L2 	& 	- 	& 	$2.91^{+1.45}_{-3.35}$ 	& 	$3.23^{+1.69}_{-3.45}$ 	& 	& 	- 	& 	$3.08^{+1.55}_{-3.29}$ 	& 	$3.14^{+1.58}_{-3.23}$ 	\\
L3 	& 	- 	& 	$2.80^{+1.35}_{-3.26}$ 	& 	$3.18^{+1.66}_{-3.47}$ 	& 	& 	- 	& 	$3.16^{+1.66}_{-3.53}$ 	& 	$3.17^{+1.64}_{-3.41}$ 	\\
L4 	& 	- 	& 	$3.20^{+1.67}_{-3.50}$ 	& 	$3.18^{+1.62}_{-3.30}$ 	& 	& 	- 	& 	$3.16^{+1.58}_{-3.19}$ 	& 	$3.10^{+1.52}_{-3.10}$ 	\\
L5 	& 	- 	& 	$2.96^{+1.42}_{-3.11}$ 	& 	$2.96^{+1.42}_{-3.01}$ 	& 	& 	- 	& 	$3.20^{+1.69}_{-3.51}$ 	& 	$3.19^{+1.64}_{-3.35}$ 	\\
L6 	& 	- 	& 	$3.19^{+1.66}_{-3.34}$ 	& 	$3.14^{+1.58}_{-3.26}$ 	& 	& 	- 	& 	$3.14^{+1.59}_{-3.37}$ 	& 	$3.13^{+1.53}_{-3.09}$ 	\\
L7 	& 	- 	& 	$3.11^{+1.55}_{-3.12}$ 	& 	$3.04^{+1.49}_{-3.14}$ 	& 	& 	- 	& 	$3.20^{+1.62}_{-3.19}$ 	& 	$3.25^{+1.59}_{-2.99}$ 	\\
L8 	& 	- 	& 	$3.19^{+1.69}_{-3.57}$ 	& 	$3.21^{+1.66}_{-3.37}$ 	& 	& 	- 	& 	$3.13^{+1.64}_{-3.54}$ 	& 	$3.17^{+1.63}_{-3.29}$ 	\\
L9 	& 	- 	& 	$2.82^{+1.33}_{-3.20}$ 	& 	$2.77^{+1.31}_{-3.10}$ 	& 	& 	- 	& 	$3.02^{+1.49}_{-3.22}$ 	& 	$2.85^{+1.32}_{-2.86}$ 	\\
T0 	& 	- 	& 	$3.20^{+1.67}_{-3.45}$ 	& 	$3.19^{+1.65}_{-3.37}$ 	& 	& 	- 	& 	$3.13^{+1.59}_{-3.35}$ 	& 	$3.21^{+1.63}_{-3.24}$ 	\\
T1 	& 	- 	& 	$3.19^{+1.67}_{-3.52}$ 	& 	$3.22^{+1.69}_{-3.43}$ 	& 	& 	- 	& 	$3.21^{+1.68}_{-3.38}$ 	& 	$3.18^{+1.63}_{-3.33}$ 	\\
T2 	& 	- 	& 	$3.08^{+1.57}_{-3.36}$ 	& 	$3.09^{+1.56}_{-3.30}$ 	& 	& 	- 	& 	$3.16^{+1.64}_{-3.35}$ 	& 	$3.20^{+1.64}_{-3.32}$ 	\\
T3 	& 	- 	& 	$3.16^{+1.69}_{-3.67}$ 	& 	$3.18^{+1.68}_{-3.49}$ 	& 	& 	- 	& 	$3.15^{+1.67}_{-3.57}$ 	& 	$3.24^{+1.71}_{-3.52}$ 	\\
T4 	& 	- 	& 	$3.08^{+1.60}_{-3.49}$ 	& 	$3.16^{+1.64}_{-3.39}$ 	& 	& 	- 	& 	$3.19^{+1.67}_{-3.53}$ 	& 	$3.21^{+1.66}_{-3.41}$ 	\\
T5 	& 	- 	& 	$3.24^{+1.76}_{-3.67}$ 	& 	$3.29^{+1.78}_{-3.57}$ 	& 	& 	- 	& 	$3.19^{+1.67}_{-3.49}$ 	& 	$3.25^{+1.68}_{-3.45}$ 	\\
T6 	& 	- 	& 	$3.19^{+1.71}_{-3.67}$ 	& 	$3.18^{+1.70}_{-3.57}$ 	& 	& 	- 	& 	$3.16^{+1.65}_{-3.55}$ 	& 	$3.14^{+1.62}_{-3.42}$ 	\\
T7 	& 	- 	& 	$3.19^{+1.72}_{-3.67}$ 	& 	$3.48^{+1.78}_{-3.24}$ 	& 	& 	- 	& 	$3.20^{+1.66}_{-3.48}$ 	& 	$3.15^{+1.65}_{-3.38}$ 	\\
T8 	& 	- 	& 	$3.16^{+1.67}_{-3.58}$ 	& 	$3.18^{+1.67}_{-3.49}$ 	& 	& 	- 	& 	$3.20^{+1.70}_{-3.54}$ 	& 	$3.20^{+1.64}_{-3.43}$ 	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}





\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:cloud q0 entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.01}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.05}$ 	\\
L1 	& 	- 	& 	- 	& 	$7.45^{+4.10}_{-6.34}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.22}$ 	\\
L2 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.01}$ 	& 	& 	- 	& 	- 	& 	$0.01^{+0.01}_{-4.10}$ 	\\
L3 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.10}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.06}$ 	\\
L4 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.17}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.30}$ 	\\
L5 	& 	- 	& 	- 	& 	$7.45^{+3.71}_{-6.32}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.02}$ 	\\
L6 	& 	- 	& 	- 	& 	$0.01^{+0.01}_{-1.54}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.07}$ 	\\
L7 	& 	- 	& 	- 	& 	$3.50^{+3.12}_{-6.93}$ 	& 	& 	- 	& 	- 	& 	$0.01^{+0.01}_{-1.46}$ 	\\
L8 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.02}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.03}$ 	\\
L9 	& 	- 	& 	- 	& 	$5.46^{+3.37}_{-6.98}$ 	& 	& 	- 	& 	- 	& 	$5.77^{+3.30}_{-6.31}$ 	\\
T0 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.25}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.07}$ 	\\
T1 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.32}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.07}$ 	\\
T2 	& 	- 	& 	- 	& 	$0.02^{+0.02}_{-6.13}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.14}$ 	\\
T3 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.16}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.03}$ 	\\
T4 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.14}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.06}$ 	\\
T5 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.13}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.03}$ 	\\
T6 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.06}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.07}$ 	\\
T7 	& 	- 	& 	- 	& 	$1.09^{+0.31}_{-0.49}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.10}$ 	\\
T8 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.10}$ 	& 	& 	- 	& 	- 	& 	$0.00^{+0.00}_{-0.21}$ 	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}


\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:cloud a0 entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	- 	& 	- 	& 	$10.36^{+8.07}_{-34.24}$ 	& 	& 	- 	& 	- 	& 	$10.43^{+7.86}_{-30.63}$ 	\\
L1 	& 	- 	& 	- 	& 	$9.16^{+6.88}_{-30.37}$ 	& 	& 	- 	& 	- 	& 	$10.08^{+7.59}_{-31.16}$ 	\\
L2 	& 	- 	& 	- 	& 	$9.96^{+7.70}_{-34.11}$ 	& 	& 	- 	& 	- 	& 	$10.01^{+7.59}_{-30.92}$ 	\\
L3 	& 	- 	& 	- 	& 	$9.95^{+7.68}_{-34.09}$ 	& 	& 	- 	& 	- 	& 	$10.17^{+7.83}_{-33.22}$ 	\\
L4 	& 	- 	& 	- 	& 	$9.92^{+7.52}_{-31.24}$ 	& 	& 	- 	& 	- 	& 	$10.54^{+7.91}_{-30.16}$ 	\\
L5 	& 	- 	& 	- 	& 	$8.92^{+6.66}_{-28.92}$ 	& 	& 	- 	& 	- 	& 	$9.81^{+7.48}_{-31.71}$ 	\\
L6 	& 	- 	& 	- 	& 	$9.73^{+7.39}_{-30.72}$ 	& 	& 	- 	& 	- 	& 	$9.50^{+6.99}_{-27.67}$ 	\\
L7 	& 	- 	& 	- 	& 	$9.67^{+7.26}_{-29.93}$ 	& 	& 	- 	& 	- 	& 	$10.09^{+7.45}_{-27.43}$ 	\\
L8 	& 	- 	& 	- 	& 	$10.08^{+7.78}_{-33.73}$ 	& 	& 	- 	& 	- 	& 	$10.05^{+7.71}_{-32.53}$ 	\\
L9 	& 	- 	& 	- 	& 	$9.37^{+7.06}_{-30.59}$ 	& 	& 	- 	& 	- 	& 	$9.85^{+7.28}_{-28.01}$ 	\\
T0 	& 	- 	& 	- 	& 	$9.83^{+7.48}_{-32.86}$ 	& 	& 	- 	& 	- 	& 	$9.85^{+7.43}_{-30.42}$ 	\\
T1 	& 	- 	& 	- 	& 	$10.06^{+7.70}_{-33.82}$ 	& 	& 	- 	& 	- 	& 	$10.32^{+7.86}_{-31.79}$ 	\\
T2 	& 	- 	& 	- 	& 	$9.56^{+7.25}_{-31.66}$ 	& 	& 	- 	& 	- 	& 	$9.96^{+7.57}_{-30.88}$ 	\\
T3 	& 	- 	& 	- 	& 	$9.91^{+7.67}_{-35.19}$ 	& 	& 	- 	& 	- 	& 	$10.25^{+7.99}_{-35.31}$ 	\\
T4 	& 	- 	& 	- 	& 	$9.89^{+7.57}_{-32.32}$ 	& 	& 	- 	& 	- 	& 	$10.08^{+7.68}_{-32.27}$ 	\\
T5 	& 	- 	& 	- 	& 	$10.78^{+8.51}_{-36.02}$ 	& 	& 	- 	& 	- 	& 	$10.14^{+7.78}_{-32.93}$ 	\\
T6 	& 	- 	& 	- 	& 	$10.24^{+8.02}_{-34.98}$ 	& 	& 	- 	& 	- 	& 	$10.13^{+7.81}_{-33.77}$ 	\\
T7 	& 	- 	& 	- 	& 	$18.68^{+14.39}_{-35.32}$ 	& 	& 	- 	& 	- 	& 	$10.22^{+7.88}_{-33.94}$ 	\\
T8 	& 	- 	& 	- 	& 	$10.18^{+7.87}_{-34.11}$ 	& 	& 	- 	& 	- 	& 	$9.78^{+7.45}_{-31.84}$ 	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}


\begin{table*}%[!h]
%\begin{rotatetable}
\label{tab:cloud particle size entire sequence}
\caption{tbd}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
	&		&	Entire spectra	&		&		&		&	Short spectra	&	\\
\cmidrule{2-4} \cmidrule{6-8}
Object	&	cloudfree	&	grey clouds	&	nongrey clouds	&       &		cloudfree	&	grey clouds	&	nongrey clouds \\
\hline
\hline
L0 	& 	- 	& 	- 	& 	$4.99^{+1.28}_{-1.30}$ 	& 	& 	- 	& 	- 	& 	$5.00^{+1.22}_{-1.22}$ 	\\
L1 	& 	- 	& 	- 	& 	$5.04^{+1.25}_{-1.23}$ 	& 	& 	- 	& 	- 	& 	$5.05^{+1.24}_{-1.20}$ 	\\
L2 	& 	- 	& 	- 	& 	$4.98^{+1.26}_{-1.29}$ 	& 	& 	- 	& 	- 	& 	$4.99^{+1.21}_{-1.22}$ 	\\
L3 	& 	- 	& 	- 	& 	$4.99^{+1.29}_{-1.29}$ 	& 	& 	- 	& 	- 	& 	$4.99^{+1.25}_{-1.27}$ 	\\
L4 	& 	- 	& 	- 	& 	$5.00^{+1.24}_{-1.25}$ 	& 	& 	- 	& 	- 	& 	$4.99^{+1.18}_{-1.19}$ 	\\
L5 	& 	- 	& 	- 	& 	$5.03^{+1.25}_{-1.23}$ 	& 	& 	- 	& 	- 	& 	$5.02^{+1.26}_{-1.24}$ 	\\
L6 	& 	- 	& 	- 	& 	$5.02^{+1.25}_{-1.22}$ 	& 	& 	- 	& 	- 	& 	$4.98^{+1.17}_{-1.19}$ 	\\
L7 	& 	- 	& 	- 	& 	$4.91^{+1.20}_{-1.24}$ 	& 	& 	- 	& 	- 	& 	$5.01^{+1.17}_{-1.14}$ 	\\
L8 	& 	- 	& 	- 	& 	$4.99^{+1.28}_{-1.29}$ 	& 	& 	- 	& 	- 	& 	$4.98^{+1.24}_{-1.27}$ 	\\
L9 	& 	- 	& 	- 	& 	$4.87^{+1.18}_{-1.30}$ 	& 	& 	- 	& 	- 	& 	$4.91^{+1.14}_{-1.20}$ 	\\
T0 	& 	- 	& 	- 	& 	$4.99^{+1.26}_{-1.28}$ 	& 	& 	- 	& 	- 	& 	$5.01^{+1.24}_{-1.23}$ 	\\
T1 	& 	- 	& 	- 	& 	$4.98^{+1.26}_{-1.28}$ 	& 	& 	- 	& 	- 	& 	$5.01^{+1.24}_{-1.24}$ 	\\
T2 	& 	- 	& 	- 	& 	$4.99^{+1.24}_{-1.25}$ 	& 	& 	- 	& 	- 	& 	$4.98^{+1.23}_{-1.25}$ 	\\
T3 	& 	- 	& 	- 	& 	$5.00^{+1.30}_{-1.29}$ 	& 	& 	- 	& 	- 	& 	$4.98^{+1.28}_{-1.29}$ 	\\
T4 	& 	- 	& 	- 	& 	$4.99^{+1.26}_{-1.26}$ 	& 	& 	- 	& 	- 	& 	$5.01^{+1.25}_{-1.26}$ 	\\
T5 	& 	- 	& 	- 	& 	$5.07^{+1.35}_{-1.28}$ 	& 	& 	- 	& 	- 	& 	$5.01^{+1.26}_{-1.25}$ 	\\
T6 	& 	- 	& 	- 	& 	$4.98^{+1.30}_{-1.32}$ 	& 	& 	- 	& 	- 	& 	$5.00^{+1.25}_{-1.27}$ 	\\
T7 	& 	- 	& 	- 	& 	$4.95^{+0.91}_{-1.04}$ 	& 	& 	- 	& 	- 	& 	$5.01^{+1.28}_{-1.27}$ 	\\
T8 	& 	- 	& 	- 	& 	$5.00^{+1.28}_{-1.29}$ 	& 	& 	- 	& 	- 	& 	$4.97^{+1.25}_{-1.26}$ 	\\
\hline
\hline
\end{tabular} }\\
%\end{rotatetable}
\end{table*}


